An Empirical Study on Hyperparameters and their Interdependence for RL Generalization

Recent results in Reinforcement Learning (RL) have shown that agents with limited training environments are susceptible to a large amount of overfitting across many domains. A key challenge for RL generalization is to quantitatively explain the effects of changing parameters on testing performance. Such parameters include architecture, regularization, and RL-dependent variables such as discount factor and action stochasticity. We provide empirical results that show complex and interdependent relationships between hyperparameters and generalization. We further show that several empirical metrics such as gradient cosine similarity and trajectory-dependent metrics serve to provide intuition towards these results.

==> extras.tex <==

\begin{comment}
We provide a case study for time horizon $T = 1$ that underlines the optimization process in policy gradients. The gradient is normally moved into the gradient log-probability in REINFORCE \cite{reinforce}:
\begin{equation}
\nabla_{\beta}\E_{x \sim p(x | \beta) } \left[f(x) \right] = \E_{x \sim p(x | \beta)} \left[ f(x) \nabla_{\beta} \log p(x| \beta) \right]  \end{equation} In the RL case, for a long horizon, $x$ is normally a sampled trajectory, with $f(x)$ being the total reward over the entire trajectory.


Suppose instead, we used probability mixture $M(x)$, which samples from $p_{base}(x)$ with probability $\alpha$, and $p_{policy}(x|\beta)$ with probability $1-\alpha)$. Then

\begin{equation}
\nabla_{\beta} \E_{x \sim M} \left[f(x) \right] = \E_{x \sim M} \left[f(x) \nabla_{\beta}\log M(x) \right] 
\end{equation}
and
\begin{equation}
\begin{gathered}
\nabla_{\beta} \log M(x) = \nabla_{\beta} \log \left( \alpha \cdot p_{base}(x) + (1-\alpha) \cdot p_{policy}(x | \beta) \right) \\ =  \frac{(1-\alpha) \cdot p_{policy}(x | \beta)}{\alpha \cdot p_{base}(x) + (1-\alpha) \cdot p_{policy}(x|\beta)} \cdot \nabla \log p_{policy}(x | \beta)= p(\text{policy} | x ) \cdot \nabla \log p_{policy}(x | \beta) 
\end{gathered}
\end{equation}


where  $p(\text{policy} | x )$ is the probability the mixture picked the policy distribution given the output was $x$. Hence 
\begin{equation}\label{two_stoch}
\nabla_{\beta} \E_{x \sim M} \left[f(x) \right] = \alpha E_{x \sim p_{base}(x)} \left[f(x) \nabla_{\beta} \log M(x) \right] + (1-\alpha)\E_{x \sim p_{policy}(x | \beta)} \left[f(x) p(\text{policy} | x ) \nabla \log p_{policy}(x | \beta) \right] 
\end{equation}

Note that the term $E_{x \sim p_{base}(x)} \left[f(x) \nabla_{\beta} \log M(x) \right] \approx 0$ especially when $KL(p_{base} || p_{policy})$ is low, which is the case during later in training, as action probabilities become more concentrated around one action. As $\alpha \rightarrow 1$, therefore $\nabla_{\beta} \E_{x \sim M} \left[f(x) \right] \approx \alpha E_{x \sim p_{base}(x)} \left[f(x) \nabla_{\beta} \log M(x) \right] \rightarrow 0$.

Furthermore the main difference after adding stochasticity is that in the rightmost term, $f(x)$ is re-weighted with $p( \text{policy} | x )$, which can smoothen the objective function $f(x)$, especially in the case of using an averaged and noisy objective function from a minibatch $\{ \theta_{1},..., \theta_{B} \}$, where $\widehat{f}(x) = \frac{1}{B} \sum_{i=1}^{B} f_{\theta_{i}}(x)$. 

Note that we cannot purely just use a bound of the gradient norm, which captures the Lipschitz constant of the loss function, which in turn can bound the generalization gap. This is because the purpose of $\alpha$ as a regularizer is to only be used at training time, not test time, which means it is necessary to analyze the gradient direction during training.

The weight $p(\text{policy} | x)$ inherently biases the gradient - if using the infinite-minibatch true expected objective $\widehat{f}_{true}(x) = \E_{\theta}\left[f_{\theta}(x)\right]$ which in many cases is smoother and has less variance, the bias due to the weight may actually hurt performance. Inversely, low minibatch-size may raise the noise and variance of the gradient.


Thus, when assessing the dot product between gradients, we ignore the LHS term in (\ref{two_stoch}) we have: 
\begin{equation}
\begin{gathered}
DP(\alpha, \beta) = \E_{x \sim p_{policy}(x | \beta)} \left[\widehat{f}(x) p(\text{policy} | x ) \nabla \log p_{policy}(x | \beta) \right]  \cdot \E_{x \sim p_{policy}(x | \beta)} \left[f_{true}(x) \nabla \log p_{policy}(x | \beta) \right]  \\= \E_{x_{1}, x_{2} \sim p_{policy}(x | \beta)} \left[\widehat{f}(x_{1}) f_{true}(x_{2}) p(\text{policy} | x_{1} ) \left(\nabla \log p_{policy}(x_{1} | \beta) \cdot \nabla \log p_{policy}(x_{2} | \beta)  \right) \right]
\end{gathered}
\end{equation}
and 
\begin{equation}
Norm(\alpha, \beta) = \norm{\E_{x \sim p_{policy}(x | \beta)} \left[\widehat{f}(x) p(\text{policy} | x ) \nabla \log p_{policy}(x | \beta) \right] }_{2}
\end{equation}
with 
\begin{equation}
GCS(\alpha, \beta) = \frac{DP(\alpha, \beta)}{Norm(\alpha, \beta)}
\end{equation}

Since $p(\text{policy} | x_{1} )  \le 1 $, 


\end{comment}




\subsection{Probabilistic POV}
It suffices to analyze when LHS numerator $\ge$ RHS numerator with high prob. and LHS denominator $\le$ RHS denominator with high prob. and see that these probabilites intersect.
\\ \\ 
Note that the LHS's denominator $\le$ RHS's denominator for some high $p$ with probability $q_{denom}(p, m)$: the sample gradient with respect to $\beta$ will tend to zero because $\beta$ has no control over actions when under high stochasticity.
\\ \\
For the numerators, consider the case for a randomly sampled single sample $\theta$ there is a probability $q_{numerator}(p, 1)$ (which will establish a smaller tail $q_{numerator}(p,m)$ ). The LHS $\ge$ RHS is equivalent to: 
$$ \Tr \left[ \nabla R_{true}(\pi_{\beta}^{p = 0})^{T} (\widehat{\nabla} R_{\theta}(\pi_{\beta}^{p})  - \widehat{\nabla} R_{\theta}(\pi_{\beta}^{p=0}) )   \right] \ge 0 $$
Noting that for a fixed $\theta, \beta$,  $\nabla R_{true}(\pi_{\beta}^{p = 0})^{T}$ and  $\widehat{\nabla} R_{\theta}(\pi_{\beta}^{p=0})$ are therefore constants. For a single reward function and state $s$ at time $t$, $\Var{\nabla_{\beta} r_{\theta, t}(s, \pi_{\beta}^{(p)})}$ effectively is raised coordinate-wise by non-zero $p$; too high of a $p$ however, will reduce this variance because the gradient signal will be lost as the policy loses control over the reward function, showing that the above may occur.
\\ \\
The above also shows that the numerator inequality holds when is roughly within some range of $p \in (0, q_{numerator}(p, m))$, while the denominator holds generally when $p$ is in some range $(q_{denominator}(p,m))$. The variances of the same gradients in both the numerator and denominator are diminished by larger samples $m$, and hence these intervals will shrink with large $m$. 
\\ \\
Thus, $q_{denom}(p, m) +q_{numerator}(p, m)  -1 \ge 0$ is fairly high for finite $m$ and some range of $p$, implying higher gradient cosine similarities. 
\\ \\ 
We emphasize that this technique \textit{does not} smooth the loss landscape because we do not use stochasticity at test time, but rather action stochasticity aligns the training gradient with the test gradient without action stochasticity.






Note that for example, if $\pi_{\beta}(a | s) = \mathcal{N}( f_{\beta}(s), \sigma I ) $ was a simple Gaussian policy, then the random action contribution (where $p_{base}$ was $\mathcal{N}(0,I)$ ) to the policy gradient is effectively a weighted noise term:
$$ \E_{a \sim p_{base} } \left[ r(s, a) \nabla_{\beta} \log \pi (a | s) \right] =  \E_{a \sim \mathcal{N}(0,1) } \left[ r(s, a) \mathbf{1}^{T}(f_{\beta}(s) - a)  \nabla_{\beta} f_{\beta}(s)\right]$$




From the above, given the state from the sample is fixed, then the gradient direction will be determined by $\nabla_{\beta} f_{\beta}(s)$ - the purpose of the action is for scaling of the direction. However, extending this to the long $T$-horizon case, the choice of action thus scales each individual gradient contribution, and hence affects the end policy gradient direction. 

Thus, there are two contributions to the policy gradient: 1. Scaling factors of individual gradient contributions which come from the reward and log probabilities of the policy, and 2. Direction of each gradient contribution, which only comes from state sequences. 

If a random action $a$ improves reward, the scaling on the individual gradient becomes higher than had the action been chosen by the policy - e.g. $1 - \pi_{\beta}(a | s)$ is high for random actions $a$, especially as the policy becomes more confident.


If diverse states were visited, the individual gradient contributions produce different directions - 




Consider the following extreme case of a contextual bandits problem: suppose $w_{\theta}: s \rightarrow obs$ was hard to invert and high dimensional (i.e. "one-way" function) for a seed $\theta$, and suppose that the state transitions were fixed $s_{1},...,s_{T}$ - thus the only contribution for policy on the total reward is the action sequence the policy inputted.

In order for a policy $\pi_{\beta}$ to have generalized \footnote{generalization here is also the definition of regret in the contextual bandits case}, it must satisfy for some small $\epsilon \ge 0$: 
\begin{equation} \E_{\theta \sim \Theta } \left[ \sum_{t=1}^{T} r(\pi_{\beta_{obs}  }(w_{\theta}(s_{t}))) ) \right]  - \E_{\theta \sim \Theta} \left[ r( \pi_{\beta_{state}}(s_{t}))   \right] \le \epsilon \end{equation}
Then for a set of $\theta$'s and $t$'s, $|r(\pi_{\beta_{obs}}(w_{\theta}(s_{t})) ) -  r(\pi_{\beta_{state}}(s_{t}) )| \le \epsilon/T$
implying that for a set of inputs, if the reward function was injective, $\pi_{\beta_{obs}}(w_{\theta}(s)) \approx s$ is nearly the identity function, and thus achieving generalization in this setting implies inverting $w_{\theta}$ on multiple inputs. 




We rigorize this notion: 

$$ \E_{S_{train}} \left[ \sup_{\beta} \left( \frac{1}{m} \sum_{i=1}^{m} R_{\theta_{i}}(\pi_{\beta}) - \E_{\theta \sim \Theta} \left[ R_{\theta}(\pi_{\beta}) \right] \right) \right] =  $$
$$ $$




\begin{center}
    \begin{tabular}{ | l | l |}
    \hline
    BMV-Deconvolution Hyperparameters & Values \\ \hline \hline 
    Network Architecture  & (filtersize = 2, stride = 1, outchannel = 500, padding = "VALID")  \\ 
                          & (filtersize = 4, stride = 1, outchannel = 40, padding = "VALID")    \\ 
                          & (filtersize = 4, stride = 3, outchannel = 20, padding = "VALID")    \\ 
                          & (filtersize = 4, stride = 3, outchannel = 10, padding = "VALID")  \\
                          & (filtersize = 4, stride = 2, outchannel = 3, padding = "VALID") \\  \hline
    Initializer          & Orthogonal Initializer \\  \hline 
    Activation & ReLU \\ \hline
    \end{tabular}
\end{center}




\subsection{Other Variants}
It remains open to understand generalization gaps for other parts in the LQR case, analogous to reinforcement learning. The following cases hold: 

\subsubsection{Action Stochasticity}
Suppose the policy took a random output $K_{random}$ with probability $p$.

Then this is equivalent to: 
$$ P_{K}^{(rand)} = Q + p \left(K_{true}^{T}RK_{true}+ (A - BK)^{T} P_{K}^{(rand)}(A-BK_{true}) \right) $$ $$ + (1-p) \E_{K_{random}} \left[K_{random}^{T}RK_{random}+ (A - BK_{random})^{T} P_{K}^{(rand)}(A-BK_{random}) \right] $$

\subsubsection{$\gamma$}
This is also equivalent to the following, since the reward matrices $Q, R$ are scaled by $\gamma$: 

$$ P_{K}^{(\gamma)} = K^{T}RK + Q + \gamma (A-BK)^{T}P_{K}^{(\gamma)} (A-BK) $$


\begin{compactitem}
\item Motivated by the "inversion framework", is it possible to recover a supervised classifier from a generalized RL agent? (e.g. if an agent generalized on a dataset with a particular reward function, can the agent be used to predict this reward function in a supervised fashion after freezing its weights?)
\item If network regularization affects the Lipschitz constant on the policy output, how does this specifically translate to the Lipschitz constant on the total horizon reward in an environment? What is the correct "complexity measure" of a convolutional policy in RL and how do we establish meaningful generalization bounds in RL?
\item Similar to the spirit of auxiliary parameters such as $\gamma$ and stochasticity, which auxiliary rewards (e.g. novelty and exploration rewards, game score bonuses) improve or decrease the generalization performance? 
\end{compactitem}

==> related_works.tex <==

\section{Related Work}
Many types of issues in robustness and overfitting, have recently been witnessed on many datasets, but some solutions have also been proposed in RL - these include: 
\begin{compactitem}
\item Overfitting to objects \cite{videobackground} and determinism \cite{brute} in pixel-based Atari \cite{atari}, and methods such as regularization \cite{coinrun}, domain randomization/data augmentation \cite{domain_randomization}, and stochasticity. 
\item Brittle policies \cite{robust_adversarial_rl}, \cite{simplicity} in control such as Mujoco, and solutions such as using simple linear policies or adversarial noise.
\item Memorization of rewards \cite{dissection} in various GridWorlds \cite{overfittingRL}, sidescrollers/random mazes \cite{coinrun}, and also more complex environments such as Gym-Retro \cite{learnfast}.
\end{compactitem}
Currently a drawback to these techniques is a lack of depth in understanding their effects on the policy or during training. Some theoretical work has been made on RL to address this deficit - for instance, on Lipschitz continuity of a policy \cite{lipschitz}, smoothness of training landscape due to entropy \cite{entropy_regularization}, $\gamma$'s effect on the size of optimal policies \cite{dependencehorizon}. However, on larger and complicated datasets such as CoinRun, there is more progress to be made on understanding the effects of RL techniques.

